NeuKron: Constant-Size Lossy Compression of Sparse Reorderable Matrices and Tensors

Many real-world data are naturally represented as a sparse reorderable matrix, whose rows and columns can be arbitrarily ordered (e.g., the adjacency matrix of a bipartite graph). Storing a sparse matrix in conventional ways requires an amount of space linear in the number of non-zeros, and lossy compression of sparse matrices (e.g., Truncated SVD) typically requires an amount of space linear in the number of rows and columns. In this work, we propose NeuKron for compressing a sparse reorderable matrix into a constant-size space. NeuKron generalizes Kronecker products using a recurrent neural network with a constant number of parameters. NeuKron updates the parameters so that a given matrix is approximated by the product and reorders the rows and columns of the matrix to facilitate the approximation. The updates take time linear in the number of non-zeros in the input matrix, and the approximation of each entry can be retrieved in logarithmic time. We also extend NeuKron to compress sparse reorderable tensors (e.g. multi-layer graphs), which generalize matrices. Through experiments on ten real-world datasets, we show that NeuKron is (a) Compact: requiring up to five orders of magnitude less space than its best competitor with similar approximation errors, (b) Accurate: giving up to 10x smaller approximation error than its best competitors with similar size outputs, and (c) Scalable: successfully compressing a matrix with over 230 million non-zero entries.

==> 010introduction.tex <==
A matrix is \textit{sparse} if a large portion of entries in it are zero.
Sparse matrices, \blue{which can also be regarded as adjacency matrices of bipartite graphs,}  naturally represent many types of data from various domains, including the following examples:

\begin{figure}[t]
    \centering
    \subfigure[Compression Quality]{
        \centering
        \includegraphics[width=0.4\linewidth]{figures/tradeoff_special.pdf}
    }
    \subfigure[Linear Scalability]{
        \centering
        \includegraphics[width=0.4\linewidth]{figures/scalability_special.pdf}
        \label{fig:effect_init}
    }
    \vspace{-1mm}
    \caption{\label{fig:intro}\method provides the best trade-off between compressed size and approximation error, with linear scalability. See Section~\ref{sec:experiments} for detailed experimental settings.} 
\end{figure}

\begin{itemize}[leftmargin=*]
\item \textbf{Search Engines}: Document-keyword matrices represent how many times each document contains each keyword \cite{liu2009bbm}. User-ad matrices indicate how many times each user clicked each ad \red{given} by search engines \cite{sidana2017kasandr}.
The adjacency matrices of web graphs represent hyperlinks between documents~\cite{boldi2004webgraph}.
\item \textbf{E-commerce}: User-item matrices represent how many times each user purchased each item  \cite{he2016ups, mcauley2012learning}.
\item \textbf{Social Media}: The adjacency matrices of social networks indicate \red{friendship} between users~\cite{dhulipala2016compressing,shin2019sweg}. User-group matrices indicate which user belongs to each group~\cite{yang2012defining}.
\item \textbf{Bibliography}: Author-paper matrices represent who authored each paper~\cite{Sinha-2015-MAG}. %Co-authorships between authors are represented as adjacency matrices of collaboration networks~\cite{yang2012defining}.
The adjacency matrices of collaboration networks represent co-authorships between authors~\cite{yang2012defining}.
\end{itemize}
\vspace{-2mm}

\blue{Despite their sparsity, many real-world matrices  require considerable space.
Examples include user-ad matrices~\cite{ting2018count} and the adjacency matrices of web graphs~\cite{boldi2004webgraph} with billions of rows or columns; and keyword-document matrices \cite{liu2009bbm} and the adjacency matrices of online social networks \cite{dhulipala2016compressing,shin2019sweg} with tens of billions of non-zeros.} %billions or tens of billions of non-zero entries.

Compression of such large sparse matrices becomes important as smartphones and IoT devices become popular. 
Such memory-limited mobile devices are often required to process a large amount of data without sending them to clouds or servers, due to potential privacy risks \cite{konevcny2016federated}.
Moreover, as the size of large-scale matrices grows rapidly, storing them is challenging also in desktops and servers \cite{shin2019sweg,dhulipala2016compressing,beutel2015accams}, and for federate learning, compressing matrices is required to reduce communication costs \cite{nam2022fedpara}.
As a result, a large number of lossy matrix-compression techniques \cite{sun2007less,beutel2015accams,drineas2006fast}  have been developed over the last few decades.

\begin{comment}
Directly accessing data on a mobile device is efficient in terms of time and network cost.
In particular, allocating a matrix on memory is the fastest way to access data since it does not require any disk I/O.
This is not enough for saving sparse matrices with several hundreds of millions of non-zero entries.
The quality of content distribution networks (CDNs) highly depends on the bandwidth between servers and clients \cite{yeo2018neural}.
Transferring sparse matrices in the conventional form suffers from a low bandwidth.
For these reasons, compressing a sparse matrix into a constant number of parameters is essential.
\end{comment}
\begin{comment}
However, concisely storing those data still requires memory proportional to the number of non-zero entries, and the required memory capacity may be very large depending on the size of the data. 
For example, the Netflix Prize dataset [], released 15 years ago, contains about 100M ratings in its user-item matrix. Also, the number of links in the web graph has reached hundreds of billions \cite{}.
Lossy but more efficient compression of sparse matrices is required in the sake of edge-computing and data transfer \cite{ting2018count}.
\end{comment}

To the best of our knowledge, existing lossy-compression methods for sparse matrices create outputs whose sizes are at least linear in the numbers of rows and columns of the input matrix.
For example, given an $N$-by-$M$ matrix $\mathbf{A}$ and a positive integer $K$, truncated singular value decomposition (T-SVD) \cite{eckart1936approximation,stewart1993early} outputs two matrices of which the numbers of entries are $O(KN)$ and $O(KM)$.
Recent methods \cite{drineas2006fast,sun2007less,beutel2015accams} have the same limitations, while they provide a better trade-off between space and information loss than T-SVD. 

Can we compress a matrix into a constant-size space, which can even be smaller than the number of rows and columns? % whose size -> which
In this paper, we exploit the fact that \textbf{many real-world sparse matrices are \textit{reorderable}}, i.e., the rows and columns of the matrices can be arbitrarily ordered.\footnote{\label{footnote:ex} A matrix is \textit{non-reorderable} if the orders of rows and columns in it convey information. For example, images and multivariate time series are non-reorderable matrices since the orders of rows and columns in them indicate spatial and temporal adjacency.}
All of the matrices discussed in the first paragraph, \blue{which are essentially bipartite graphs (nodes of one type correspond to rows, and  nodes of the other type correspond to columns)}, are reorderable.
For example, in the case of user-item matrix built based on e-commerce data, which user (item) comes next to which user (item) does not matter.
Our key idea is to order rows and columns to facilitate our model to learn and exploit meaningful patterns in the input matrix for compression. %our machine learning model -> our model
      
Specifically, we present \method, a constant-size lossy compression method for sparse reorderable matrices.
%\method consists of a machine learning model and novel training schemes.
\red{It} consists of a machine-learning model and novel training schemes.
The model generalizes the Kronecker power and enhances its expressive power using a \red{recurrent neural network} with a constant number of parameters. 
Consider \red{an} $N$-by-$M$ matrix with $L$ non-zeros, where $N \!\leq \!M$ without loss of generality. The model and the training schemes are designed carefully so that each training epoch takes $O(M+L\log M)$ time, and after training, the approximation of each entry can be retrieved in $O(\log M)$ time. 
Note that the time complexity of training depends \red{only on the number of non-zeros} instead of all entries.

In addition, we extend \method for lossy-compression of sparse reorderable tensors while maintaining its strengths. Tensors (i.e., multi-dimensional arrays) generalize matrices to  higher dimensions, and in other words, matrices are 2-order tensors. 
Sparse tensors have been used widely for various purposes, including context-aware recommender systems \cite{karatzoglou2010multiverse} and knowledge base completion \cite{lacroix2018canonical}), and for lossy compression of them, tensor decomposition methods (e.g., CP \cite{carroll1970analysis,bader2008efficient} and Tucker \cite{tucker1966some,bader2008efficient}) have been developed.

For evaluation, we perform extensive experiments using ten real-world matrices \blue{(spec., bipartite graphs)} and tensors. 
As highlighted in Figure~\ref{fig:intro}, the results reveal the following advantages of \method:

\vspace{-2mm}
\begin{itemize}[leftmargin=*]
    \item \textbf{Compact:} Its output is up to \textbf{5 orders of magnitude smaller} than \red{competitors' with similar approximation error.}
    \item \textbf{Accurate:} It achieves up to \textbf{10.1$\times$ smaller approximation error} than its best competitors that give similar-size outputs.
    \item \textbf{Scalable:} Its running time is \textbf{linear} in the number of non-zero entries, and it successfully compresses matrices with \textbf{over 230 millions of non-zero entries} on commodity GPUs. %\textbf{hundreds of millions of non-zero entries} on commodity GPUs. 
\end{itemize}
\vspace{-2mm}

\smallsection{Reproducibility}
The code and datasets are available at \supplelink.

\smallsection{Remarks on non-reorderable matrices}
While we focus on reorderable matrices throughout this paper, \method can also be applied to non-reorderable matrices if the mapping between the original and new orders of rows and columns are stored additionally. 
\textbf{Even with this extra space requirement}, which is linear in the number of rows and columns, \textbf{\method still gives a better trade-off} between size and approximation error than its competitors, as shown in Figure~\ref{fig:appdix:trade-off} of Appendix~\ref{app:non_reorder}.

% Twitch: 6525763600 / (31244 + 48290559.4565) => 135.04x

\smallsection{Roadmap} In Section \ref{sec:related}, we survey some related works. In Section~\ref{sec:preliminaries}, we give notations and the problem definition. In Section~\ref{sec:method}, we present \method and analyze its complexity. In Section~\ref{sec:tensor}, we describe its extension for tensor compression.
In Section \ref{sec:experiments}, we review experimental results.
Lastly, in Section \ref{sec:conclusion}, we provide conclusions.
\vspace{-1mm}


==> 020related.tex <==
In this section, we review lossy-compression methods for matrices and tensors. We further divide matrix compression methods into (a) factorization-based ones, (b) co-clustering-based ones, and (c) Kronecker-product-based ones.%(a) factorization-based methods, (b) co-clustering-based methods, and (c) Kronecker-product-based methods.

\smallsection{Factorization-based matrix compression}
Given a matrix $\mathbf{A} \in \mathbb{R}^{M \times N}$, singular value decomposition (SVD) \cite{golub1971singular} decomposes $\mathbf{A}$ into $\mathbf{U}\Sigma \mathbf{V}^T$ where $\mathbf{U} \in \mathbb{R}^{M \times R}$, $\mathbf{V} \in \mathbb{R}^{N \times R}$, $\mathbf{\Sigma}$ is a diagonal matrix with its singular values, and $R$ is its rank.
Truncated SVD (T-SVD) \cite{eckart1936approximation,stewart1993early} outputs the $K$ $(\leq R)$ largest singular values and the corresponding vectors of $\mathbf{U}$ and $\mathbf{V}$ from which the rank-$K$ approximation of $\mathbf{A}$ best in terms of the Frobenius norm  can be obtained \cite{stewart1993early}.
It should be noted that its outputs have $O(K(M+N))$ real values.
There are several variants of T-SVD for sparse matrices.
CUR decomposition \cite{drineas2006fast} approximates given $\mathbf{A} \in \mathbb{R}^{M \times N}$ by $\mathbf{CUR}$, where $\mathbf{C} \in \mathbb{R}^{N \times K}$ and $\mathbf{R} \in \mathbb{R}^{K \times M}$ are created by sampling $K$ columns and rows from $\mathbf{A}$, and $\mathbf{U}$ is calculated from $\mathbf{C}$ and $\mathbf{R}$. If $\mathbf{A}$ is sparse, $\mathbf{C}$ and $\mathbf{R}$ are also likely to be sparse, %\blue{so the method requires less space than T-SVD.} 
requiring less space than T-SVD.
Compact matrix decomposition (CMD) \cite{sun2007less} keeps only unique columns and rows in $\mathbf{C}$ and $\mathbf{R}$ for further efficiency. %improvement.

% 오타 수정
\smallsection{Co-clustering-based matrix compression} ACCAMS and bACCAMS~\cite{beutel2015accams} use an additive combination of small co-clusterings to approximate a given matrix. While the numbers of parameters of them are linear in the number of rows and columns,
they produce intermediate results whose size is linear in the number of (potentially zero) known entries.
Thus, they are not proper when most entries are known but zero, as in matrices considered in this work.

\smallsection{Kronecker product-based matrix compression}
% 오타수정
The adjacency matrix of a Kronecker graph \cite{leskovec2005realistic} is a Kronecker power of a fixed seed matrix (e.g., $2$-by-$2$ matrix).
\kronfit~\cite{leskovec2007scalable, leskovec2010kronecker} searches for a seed matrix whose Kronecker power approximates the adjacency matrix of a given graph.
While \kronfit is designed for adjacency matrices, it can be easily extended to matrices of any size, and the output seed matrix can be considered as a constant-size lossy compression of a given matrix.
However, the approximation error is considerable, even when the seed matrix is large, due to the inflexibility of the Kronecker product, as shown in Section~\ref{sec:exp:model}.

\smallsection{Tensor compression} 
CP decomposition (CP)~\cite{carroll1970analysis} and Tucker decomposition (Tucker)~\cite{tucker1966some} generalize
the aforementioned T-SVD to higher-order tensors.
They approximate a given tensor using the sums and products (e.g., outer product and $n$-mode product) of much smaller low-rank tensors and matrices, which can be considered as a lossy compression of the given tensor.
%There exist quasi-optimal methods for Tucker, i.e., the error of the resulting approximation is comparable to the best possible~\cite{vannieuwenhoven2012new, hackbusch2012tensor}. 
There exist quasi-optimal methods for Tucker~\cite{vannieuwenhoven2012new, hackbusch2012tensor}. \blue{Moreover, efficient CP and Tucker methods for sparse tensors have been developed \cite{bader2008efficient}.
For lossless compression of sparse tensors, compressed sparse fiber~(CSF)~\cite{smith2015splatt, smith2015tensor} is available.}

\smallsection{Other related works}
\blue{Unipartite-graph summarization algorithms \cite{lee2020ssumm,lefevre2010grass,riondato2017graph} can be used for compressing adjacency matrices of unipartite graphs, while they cannot be directly applied to weighted and/or non-symmetric matrices, which we aim to compress.}
Matrix sketching methods replace a given large matrix with a more compact matrix that follows the properties of the input matrix, for example, by leaving only important columns (rows) of the input matrix \cite{drineas2006fast,drineas2008relative}.
These methods, however, cannot be applied to our problem (i.e., Problem~\ref{prob} in Section~\ref{sec:preliminaries:problem}) because the entries of the input matrix cannot be estimated directly from their outputs. For federated learning, the weights of neural networks, which are typically dense matrices or tensors, can be compressed \cite{nam2022fedpara}.

% 오타 수정
Among the aforementioned ones, those that can be used for lossy compression of sparse matrices and tensors of any size (i.e., T-SVD, CUR, CMD, ACCAMS, bACCAMS, \kronfit, CP, and Tucker) are compared numerically with \method in the experiment section.


==> 030notation.tex <==
\vspace{-0.5mm}

In this section, we introduce basic concepts and give a formal problem definition.
\red{See Table~\ref{tab:notation} for common notations.}
%The frequently used notations are listed in Table~\ref{tab:notation}.

\vspace{-1.5mm}
\subsection{Notations and Concepts}
\vspace{-0.5mm}

\smallsection{Sparse reorderable matrix and tensor} 
A \textit{matrix} $\bA \in \mathbb{R}^{N \times M}$ is a 2-dimensional array with $N$ rows and $M$ columns, and real entries. 
A $D$-order \textit{tensor} $\cX \in \mathbb{R}^{N_1 \times \cdots \times N_{D}}$ is a $D$-dimensional array of size $N_1\times\cdots\times N_D$ with real entries. 
We use $a_{ij}$ or $A(i,j)$ to denote the $(i,j)$-th entry of $\bA$, and we use $x_{i_1, \cdots, i_D}$ to denote the ($i_1$, $\cdots$, $i_{D}$)-th entry of $\cX$.
We call a matrix or a tensor \textit{sparse} if the number of zero entries in it dominates the number of non-zero entries.
We call a matrix \textit{reorderable} if its rows and columns can be arbitrarily ordered. We provide some examples of reorderable matrices where the orders of rows and columns do not convey any information and some examples of non-reorderable ones (see Footnote~\ref{footnote:ex}) in Section~\ref{sec:intro}.
Similarly, we call a tensor reorderable if the indices in each mode can be arbitrarily ordered.

%A \textit{reordered} matrix $\bA^{(\pi, \phi)}$ is a representation of matrix $\bA$ with a permutation $\pi$ for rows and a permutation $\phi$ for columns.
%The permutation $\pi$ saves one to one mapping from rows of $\bA$ to rows of $\bA^{(\pi, \phi)}$, and the permutation $\phi$ saves one to one mapping from columns of  $\bA$ to columns of $\bA^{(\pi, \phi)}$. 
%The $(i,j)$-th entry of $\bA$ is identical to the $(\pi(i), \phi(j))$-th entry of  $A^{(\pi(i),\phi(j))}$.

% A \textit{reordered} tensor $\cX^{(\psi_1, \cdots, \psi_{D})}$ is a representation of tensor $\cX$ with permutations $\psi_1$, $\psi_2$, $\cdots$, $\psi_{D}$ where $\psi_i$ saves one to one mapping from indices of $i$-th dimension of $\cX$ to those of $\cX^{(\psi_1, \psi_2, \cdots, \psi_{D})}$.}

\smallsection{Approximation error} The \textit{Frobenius norm} is a function $\lVert \cdot \rVert_{F}: \mathbb{R}^{N \times M} \rightarrow \mathbb{R}$ defined as the square root of the square sum of all entries in the given matrix.
Similarly, the Frobenius norm of a tensor is defined as the square root of the square sum of all entries in the given tensor.
The \textit{approximation error} of a matrix $\reA$ that approximates $\bA$ is defined as $\lVert \bA - \reA \rVert_F^2$.
Similarly, the approximation error of $\reX$ that approximates $\cX$ is defined as $\lVert \cX - \reX \rVert_F^2$. 

\smallsection{Kronecker product and power} 
Given two matrices $\bA \in \mathbb{R}^{N \times M}$ and $\mat{B} \in \mathbb{R}^{P \times Q}$, the \textit{Kronecker product} $\bA \otimes \mat{B} \in \mathbb{R}^{NP \times MQ}$ is a large matrix formed by multiplying $\mat{B}$ by each element of $\bA$, i.e.,
\vspace{-2mm}
$$
\bA \otimes \mathbf{B} := %\triangleq 
\begin{bmatrix}
a_{11} \mathbf{B} & a_{12} \mathbf{B} & \cdots & a_{1M}\mathbf{B} \\
a_{21} \mathbf{B} & a_{22} \mathbf{B} & \cdots & a_{2M}\mathbf{B} \\
\vdots & \vdots & \ddots & \vdots \\
a_{N1} \mathbf{B} & a_{N2} \mathbf{B} & \cdots & a_{NM}\mathbf{B}
\end{bmatrix}.
$$
We denote the $l$-th \textit{Kronecker power} of $\bA$ as $\kpower{\bA}{l}$, where $\kpower{\bA}{l}=\kpower{\bA}{(l-1)} \otimes \bA$ and $\kpower{\bA}{1}=\bA$.
\vspace{-2mm}

\subsection{Problem Definition}
\label{sec:preliminaries:problem}
The constant-size lossy matrix compression problem that we address in this paper is defined in Problem~\ref{prob}.
\noindent It should be noted that the given constant $k$ can be even smaller than $N$ and $M$.
The problem of \textit{constant-size lossy compression of a sparse reorderable tensor} can be defined by simply replacing the matrix $\bA$ with a tensor $\cX$ and $\lVert\bA - \reA\rVert_F^2$ with $\lVert \cX - \reX \rVert_F^2$.

\vspace{0.5mm}
\noindent\fbox{%
        \parbox{0.975\columnwidth}{%
        \vspace{-2mm}
        \begin{problem}\label{prob}
\textsc{\normalfont{(Constant-size Lossy Compression of a Sparse}} \textsc{\normalfont{Reorderable Matrix)}} 
\begin{itemize}[leftmargin=*]
    \item \textbf{Given:} (1) a sparse and reorderable matrix $\bA \in \mathbb{R}^{N \times M}$, \\
    \indent \hspace{9mm} (2) a constant $k= O(1)$,
     % and a bound $\bound$ on a model size
    \item \textbf{Find:} a model $\model$ %with parameters $\params{\bA}$ %, such that the size of  $\params{\bA}$ is small enough, $| \params{\bA}| \ll max(N, M)$
    \item \textbf{to Minimize:} the approximation error 
        $\lVert\bA - \reA\rVert_F^2$, where $\reA$ is the matrix approximated from $\model$.
    \item \textbf{Subject to:}
    the number of parameters in $\model$ is at most $k$.
\end{itemize}
\end{problem}
        \vspace{-2mm}
        }%
        %\vspace{2mm}
    }
%\vspace{1mm}

%\vspace{1mm}
\begin{table}[t]
    \centering
    \caption{Frequently-used notations}
    \label{tab:notation}
    \scalebox{0.85}{
    \begin{tabular}{c|l}
        \toprule
        \textbf{Symbol} &  \textbf{Definition} \\
        \midrule
        $\bA\in \mathbb{R}^{N \times M}$ & an $N$-by-$M$ sparse matrix \\
        $a_{ij}$ or $\bA(i, j)$ & ($i$, $j$)-th entry of $\bA$ \\
        $\bA_{i,:}$, $\bA_{:,i}$ & $i$-th row of $\bA$, $i$-th column of $\bA$ \\
        %$\pi$, $\phi$ & permutation for rows and columns\\
        %$\bA^{(\pi, \phi)}$ & reordered version of $\bA$ by $\pi$ and $\phi$\\
        \midrule
        $\cX\in \mathbb{R}^{N_1 \times \cdots \times N_{D}}$ & tensor \\
        $D$ & order of $\cX$ \\
        $x_{i_1, \cdots, i_D}$ & ($i_1$, $\cdots$, $i_D$)-th entry of $\cX$ \\
        %$\psi_i$ & permutation for $i$-th dimension of tensor \\
        %$\cX^{(\psi_1, \psi_2, \cdots, \psi_{D})}$ & reordered version of $\cX$\\
        \midrule
        $\text{nnz}(\bA)$, $\text{nnz}(\cX)$ & number of non-zero entries in $\bA$ and $\cX$ \\
        $\fnorm{\bA}, \fnorm{\cX}$ & Frobenius norm of $\bA$ and $\cX$\\
        %$\oplus$ & XOR operation\\
        $\otimes$ & Kronecker product \\
        $\kpower{\bA}{l}$, $\kpower{\cX}{l}$ & $l$-th Kronecker power of $\bA$ and $\mathbf{\cX}$ \\
        $\model$ & a \method model which compresses $\bA$ and $\cX$ \\
        %$\model, \model{\cX}$ & model that compresses $\bA$ and $\cX$ \\
        %$\params$ & parameters of $\model$ \\
        %$\params{\bA}, \params{\cX}$ & parameters of $\model$ and $\model{\cX}$ \\
        $\reA$, $\reX$  & approximated matrix and tensor of $\bA$ and $\cX$ by $\model$ \\
        %$\reX$ & approximated tensor of $\cX$ by $\model$ \\
        $q$ & a parameter for the scale of model outputs \\
        $h$ & hidden dimension in LSTM \\
        $[n]$ & a set of integers from $1$ to $n$ (i.e., $\{1, 2, \cdots, n\}$) \\
        \bottomrule
    \end{tabular}
    }
    %\vspace{-1mm}
\end{table}

==> 060conclusion.tex <==
In this work, we focus on compressing sparse reorderable matrices and tensors, including  the adjacency matrices of bipartite graphs, into a constant-size space. 
%We propose \method, a scalable auto-regressive model which generalizes Kronecker graph, and the novel training strategies for \method. 
% Through experiments on ten real-world datasets, we show the contributions as follows:
Our contributions are three-fold:
\begin{itemize}[leftmargin=*]
    \item \textbf{Compact yet Accurate Method:} We proposed \method, which lossily compresses matrices and fixed-order tensors of any size with a constant number of parameters. %theoretically
   \method provided an output that is up to five orders of magnitude smaller than the outputs of the best competitors when the approximation errors in them are similar (Figure~\ref{fig:compression}). % deletion: in our experiments
    
     \item \textbf{Theoretical Analysis:} We carefully designed \method so that, for sparse reorderable matrices and fixed-order tensors of any size (a) the number of parameters is constant, (b) each entry is approximated in a logarithmic time, and (c) the model is fitted to an input in time proportional to the number of non-zero entries in it. We proved these desirable properties (Theorems~\ref{theorem:query}-\ref{thm:num_params}).
     % 원래 thm:num_params_t였음.
     
%    its best competitors with similar space requirements and shows comparable performance to the previous works consuming up to five orders of magnitude times more parameters. %empirically
    % We propose \method, which generalizes Kronecker product to compress matrices and tensors while keeping a constant number of parameters. %theoretically
    % As mentioned in Section~\ref{sec:exp:model}, \method outperforms the baselines with similar space requirements and shows comparable performance to the previous works consuming up to five orders of magnitude times more parameters. %empirically
    
    \item \textbf{Extensive Experiments:}
    Through extensive experiments on $10$ real-world datasets %\change{which include bipartite graphs and hypergraphs}
    , we demonstrated the effectiveness and scalability of \method (Figures~\ref{fig:compression} and \ref{fig:scalability}).
    %(Figures~\ref{fig:compression}, \ref{fig:scalability} and \ref{fig:scalability_t}). 
    We also analyzed its approximation error and the effects of its components (Figures~\ref{fig:ablation}, \ref{fig:reconst}, and \ref{fig:q5}).
    Especially, we showed that \method successfully compressed a matrix with up to $230$ millions of non-zero entries.
    % \item \smallsection{Effective Training Strategies} 
    % We carefully design the model so that the loss and the gradient can be computed in efficient manners given a sparse matrix.
    % In addition, we propose a novel optimization method for ordering rows and columns that exploits similarity between them,
    % %theoretically
    % We verify that our training strategies and the design of the model output more accurate compression, compared to the variants without min-hashing or other components in Section~\ref{sec:exp:method}. 
    % Also, we show that \method equipped with the strategies compresses the matrices with up to $230$ millions non-zero entries, and its running time increases linearly to the number of non-zero entries in Section~\ref{sec:exp:scalability}. %empirically 
    
    % \item \smallsection{Theoretical Analysis} 
    % \item \smallsection{Extensive Experiments} 
    
\end{itemize}
\smallsection{Reproducibility}
The code and datasets used are
available at~\supplelink.
%Our proposed design can express more diverse representations while extending self-similarity, one of the main properties of Kronecker graph. Also, our design has a constant number of parameters regardless of the size of target matrix. We evaluate the empirical performance of \model in Section 5. We check that \model outperforms all baselines in all datasets and is well trained on a 100 million scale dataset which cannot be run on some baselines.
